You Only Crash Once v2: Perceptually Consistent Strong Features for One-Stage Domain Adaptive Detection of Space Terrain

The in-situ detection of planetary, lunar, and small-body surface terrain is crucial for autonomous spacecraft applications, where learning-based computer vision methods are increasingly employed to enable intelligence without prior information or human intervention. However, many of these methods remain computationally expensive for spacecraft processors and prevent real-time operation. Training of such algorithms is additionally complex due to the scarcity of labeled data and reliance on supervised learning approaches. Unsupervised Domain Adaptation (UDA) offers a promising solution by facilitating model training with disparate data sources such as simulations or synthetic scenes, although UDA is difficult to apply to celestial environments where challenging feature spaces are paramount. To alleviate such issues, You Only Crash Once (YOCOv1) has studied the integration of Visual Similarity-based Alignment (VSA) into lightweight one-stage object detection architectures to improve space terrain UDA. Although proven effective, the approach faces notable limitations, including performance degradations in multi-class and high-altitude scenarios. Building upon the foundation of YOCOv1, we propose novel additions to the VSA scheme that enhance terrain detection capabilities under UDA, and our approach is evaluated across both simulated and real-world data. Our second YOCO rendition, YOCOv2, is capable of achieving state-of-the-art UDA performance on surface terrain detection, where we showcase improvements upwards of 31% compared with YOCOv1 and terrestrial state-of-the-art. We demonstrate the practical utility of YOCOv2 with spacecraft flight hardware performance benchmarking and qualitative evaluation of NASA mission data.

==> figs/inst_advcont.tex <==
\begin{figure*}
    \centering
    \includesvg[width=\textwidth]{figs/inst_advcont.svg}
    \caption{Contrastive and adversarial region-of-interest-based (ROI) loss configurations for $\inst$. Detected regions are extracted from feature maps (ROI Extraction) and are either similarity-learned directly ($\mathcal{L}_{\text{Contrastive}}$) or adversarially through discriminators on mean cluster embeddings ($\mathcal{L}_{\text{Adversarial}}$). An additional perception loss ensures consistency between feature maps before detections are made ($\mathcal{L}_{\text{Perceptual}}$) while a learnable filter highlights the most relevant and impactful of these maps (Top-K Selection).}
    \label{fig:inst-advcont}
\end{figure*}
% The purple boxes highlight each method, with $\mathcal{L}_{\text{Contrastive}}$ and $\mathcal{L}_{\text{Adversarial}}$ being mutually exclusive.

==> figs/inst_fmap.tex <==
\begin{figure*}
    \centering
    \includesvg[width=\textwidth]{figs/inst_fmap.svg}
    \caption{Loss configurations for $\inst$ based on activation clustering. Unlike ROI-based $\inst$ (\autoref{fig:inst-advcont}), the set of source and target object-level feature maps are clustered into groups of either classes + 1 (YOCOv1~\cite{yoco}), foreground (FG)/background (BG) (K-Means), or strong pixel pooled (SPP) using self-attention. Mean cluster groups (group discrimination) from YOCOv1 and K-Means feed a discriminator loss ($\mathcal{L}_{\text{Adversarial}}$) while the resulting SPP feature map feeds this loss directly.}
    \label{fig:inst-fmap}
\end{figure*}

==> sections/_notes_eval.tex <==
% Although these are sim-to-sim benchmarks, we view the quantitative experiments as a comprehensive overview of the VSA procedures (and UDA in general) as each dataset is visually distinguishable and thus we expect the feature distribution to vary. 

==> sections/_notes_intro.tex <==
The detection of celestial surface terrain is vital for autonomous spaceflight applications, including Terrain Relative Navigation (TRN), Entry, Descent, and Landing (EDL), hazard and composition analysis, and science data acquisition. Traditional terrain detection methods are constrained by the limited computational power of onboard radiation-hardened systems, requiring extensive \textit{a priori} imaging with detections processed offline by human operators~\cite{nft1,nft2,retina,m2020lvs}. Although demonstrated successfully on recent flagship missions including the landing of the Mars Perseverance Rover~\cite{m2020lvs} and small-body touch-and-go by OSIRIS-REx~\cite{nft1,nft2}, these approaches inflate mission timelines and costs, cannot generalize on new instances of terrain or perform detections in-situ, and suffer from poor data processing rates. With the recent advent of novel hardware architectures that can accelerate the inference of learning-based algorithms~\cite{sclearn}, more advanced state-of-the-art computer vision approaches, such as object detection techniques, can be deployed to alleviate these issues with real-time performance~\cite{profiling} and robust recognition techniques~\cite{mars}.

However, there is a significant bottleneck in the training of current object detection methods. Many techniques remain supervised learning approaches, requiring vast amounts of labeled training data to effectively learn how to detect and classify objects of interest. This poses a significant challenge for spaceflight applications, as celestial surface terrain imaging is scarce, and ground truth labels are either difficult to obtain or entirely unavailable, particularly for missions targeting previously unexplored environments. When a similar challenge is faced in terrestrial vision tasks, Unsupervised Domain Adaptation (UDA) is employed to train the model on a distinct, cheaper-to-acquire data distribution while adapting the model's learned capacity to the target environment. Such a technique is well-suited for the space domain, where photorealistic simulations or lower-resolution mission data can be used as a starting point.

The application of UDA to imaging in space environments, particularly celestial surfaces, is non-trivial, however. Difficult illumination conditions, textureless regions, and similarity in feature spaces are highly prevalent due to the unstructured nature of the space terrain~\cite{slamprob1,slamprob2,slamprob3,mht}, which makes distribution alignment more demanding. A promising approach to achieve UDA in such scenarios is the employment of Visual Similarity-based Alignment (VSA). Originally proposed for two-stage detectors~\cite{visga}, VSA aggregates object features into instance-level groups by visual appearance before minimizing the distribution shift. Such an approach does not operate on class labels or classifications of predicted target detections, which may be incredibly noisy and incorrect as the training evolves. 
% This permits a robust alignment strategy that can lessen the distribution alignment difficulty with challenging space data. 
Two-stage detectors are not suitable for in situ spacecraft inference, however, as these models are generally too large for the latest generation of spacecraft accelerators~\cite{sclearn} where one-stage, lightweight models are required~\cite{profiling}.
% where object detection algorithms are currently limited to one-stage methods for real-time or near-real-time processing rates~\cite{profiling}. 
Previous attempts at adapting VSA to one-stage algorithms have been largely successful through the \textit{You Only Crash Once} (YOCO~\cite{yoco}) framework, although degraded performance is still observed in scenes of overly smooth and similar terrain features, such as imagery of the Mars surface captured at high altitudes.

In this work, we propose the next rendition of the YOCO framework adaptable to a broader set of one-stage architectures, offering an improved VSA formulation for real-time, onboard, and in-situ terrain surface detection on challenging planetary, moon, and small-body scenes. We specifically target improvements in the presence of textureless regions and varying illumination conditions, incorporating recent ideas in image generation to bridge the distribution gap. We explore the full spectrum of VSA techniques including instance and intra-feature-based clustering methods in adversarial and contrastive learning settings, discovering correlations between clustering technique and type of terrain. Through rigorous quantitative and qualitative analysis on both simulated and real-world data, we demonstrate our improved VSA formulation and present improved accuracy by upwards of 31\% to YOCOv1 and terrestrial state-of-the-art methods. 

==> sections/_notes_method.tex <==
In this work, our objective is to develop a lightweight object detection algorithm capable of running onboard current spacecraft hardware without the need for custom acceleration. The algorithm is designed to be generalizable across diverse terrain features and can be effectively trained using low-cost synthetic data through unsupervised domain adaptation (UDA) to achieve high performance in the target environment. We extend the YOCOv1 framework by incorporating alternative VSA strategies which yield superior performance depending on the specific environmental conditions and feature structures encountered. Our primary contributions beyond YOCOv1 are: (1) enhanced VSA schemes and configurations, including improved region-of-interest (ROI)-based learning and an exploration of alternative feature clustering methods, and (2) architecture-agnostic design, allowing compatibility with any YOLO model variant to facilitate real-time performance considerations. 

The key idea in Adversarial Training (AT) based UDA methods is to learn domain invariant
representations by fooling a discriminator which is trained
to predict the input data domain based on the detector features. This approach is usually class-agnostic, ignoring
the features class information and focusing on domain-level
alignment. Specifically, the features Fd of domain d (d = 0
for source and d = 1 for target) is fed to the discriminator
D which predicts the domain of the extracted features. The
discriminator is trained by minimizing the cross-entropy
loss as below:

\textbf{\textit{REWRITE FROM VISGA:}} Since we want to adapt the features of the two domains to be indistinguishable by the discriminator, we have to maximize the loss in Equations (2) w.r.t the features $F_d$. This
is achieved by incorporating a gradient reverse layer (GRL)
[13], before features are input to the discriminator.

\textbf{\textit{REWRITE FROM AERO PAPER:}} Prior works that employ multi-scale discriminators [27, 28]
improve adversarial loss through the inclusion of a featurematching component based on this discriminator. Features
are extracted from multiple layers of the discriminator on real
and synthesized images and the features are aligned by minimizing the mean absolute error. This helps stabilize training as the generator is forced to produce natural, realisticlooking features across the different scales. Given each $k$ scale discriminator, the feature matching loss $\pc$ is calculated as:

Contrastive and adversarial region-of-interest-based (ROI) loss configurations for $\inst$. Detected regions are extracted from feature maps (ROI Extraction) and are either similarity-learned directly ($\mathcal{L}_{\text{Contrastive}}$) or adversarially through discriminators on mean cluster embeddings ($\mathcal{L}_{\text{Adversarial}}$). An additional perception loss ensures consistency between feature maps before detections are made ($\mathcal{L}_{\text{Perceptual}}$) while a learnable filter highlights the most relevant and impactful of these maps (Top-K Selection).

\textbf{\textit{REWRITE FROM VISGA:}} To perform similarity-based
clustering, we take as input the N proposals generated by
RPN and their fixed feature vectors denoted by $f \in \mathbb{R}^{Nxm}$.
In order to discover the main feature groups, we cluster
these features using hierarchical agglomerative clustering.
Starting bottom-up, each proposal is considered as an individual cluster. Then, at each step, the two closest clusters
according to a distance metric are merged together. We utilize cosine distance as our merging metric:

using cosine similarity enables us to pair instances which are located far from each other, but are visually similar. Merging
is stopped when dissimilarity within a cluster, as defined by
a linkage function, exceeds the cluster radius parameter $\tau$.
We apply the complete-linkage heuristic [8], which ensures
that the farthest distance of two members is smaller than $\tau$:

\textbf{\textit{REWRITE FROM VISGA}} where A, B are two sets of proposals’ features in two clusters and dist is the cosine distance. This hierarchical clustering approach allows our model to adaptively change the
number of feature groups during training, instead of having
a fixed number of cluster like in k-means. Once the clustering has converged, instances assigned to each cluster are pooled to construct a representative embedding $Z_{c_i}$:

\textbf{\textit{REWRITE FROM VISGA:}} As an alternative to AT, one can apply max-margin contrastive losses to align source and target features by leveraging the class information. The main
idea here is to push features from the same class closer and
push apart features belonging to different classes across domains. When matching a single feature vector $F_{d}^{i}$ per class $i$
in each domain $d \in (0, 1)$, the max-margin contrastive loss
takes the form:

\textbf{\textit{VISGA REWRITE:}} where C is the number of classes and m is the margin.
Since target data is unlabeled, the class prediction by the
detector is used as a pseudo-label in [44] to apply Equation (3). In our analysis, we also study the effect of ignoring
this class information. This can be achieved by considering
only two sets of vectors of cardinality $N_0$ and $N_1$, possibly
unequal number ($N_0 \neq N_1$), from source and target domains to align. To apply contrastive losses here, we make
a simple modification. Instead of matching class-specific
features across domains, we match the proposals from one
domain to the closest features (nn) of the other domain (4)
and minimize the distance between their representations (5),
as shown below:

Loss configurations for $\inst$ based on activation clustering. Unlike ROI-based $\inst$ (\autoref{fig:inst-advcont}), the set of source and target object-level feature maps are clustered into groups of either classes + 1 (YOCOv1~\cite{yoco}), foreground (FG)/background (BG) (K-Means), or strong pixel pooled (SPP) using self-attention. Mean cluster groups (group discrimination) from YOCOv1 and K-Means feed a discriminator loss ($\mathcal{L}_{\text{Adversarial}}$) while the resulting SPP feature map feeds this loss directly.

\textbf{\textit{REWRITE PTAP:}} We propose a new attention pooling based on activations’ priority which is defined as follows. To obtain the priority, we first employ a channel
attention module [35] to assign importance weights for
each channel of the feature map. Specifically, we apply
a global average pooling (GAP) [23] layer, a 1D convolution, and sigmoid function sequentially on the feature map $Fx \in RC×H×W$. Then, we compute the weighted feature map $Fw \in RC×H×W$ by:

% ==========================================================
YOCOv1 proved to be a successful step toward bolstering UDA performance in one-stage terrain detection but retains many limitations that limit the adaptation for future missions. Building upon the YOCOv1 formulation, we seek to improve and devise a VSA strategy that is applicable to a wider range of celestial environments, while simultaneously generalizing to any YOLO architecture that can promise real-time or near-real-time performance on current spacecraft hardware. 

% this work proposes novel VSA strategies that offer enhanced adaptability to diverse environmental conditions and terrain characterizations in challenging remote sensing settings in space, while simultaneously generalizing to generic one-stage detection architectures that promise real-time or near-real-time performance on current spacecraft hardware without custom mission-specific acceleration techniques. We first describe the baseline YOLO architecture and modifications for UDA in~\autoref{sec:arch}, followed by our techniques for VSA instance alignment in~\autoref{sec:inst}.


% followed by the alignment scheme for global image features in~\autoref{sec:glob}. Finally, we introduce our novel formulation of instance VSA in~\autoref{sec:inst}.

% Our novel formulation of VSA instance alignment for instance-only and full-feature schemes 

% This work aims to develop a lightweight object detection algorithm optimized for deployment on current spacecraft hardware without requiring custom accelerators. The proposed algorithm is designed to generalize effectively across varied terrain features and leverages low-cost synthetic data with UDA to achieve high performance in target environments. B

% uilding upon the YOCOv1 framework, this approach proposes novel VSA strategies that offer enhanced adaptability to diverse environmental conditions and terrain characterizations. 

% The primary contributions include: (i) improved VSA configurations, such as advanced instance-only learning and alternative feature clustering techniques, and (ii) an architecture-agnostic framework compatible with any YOLO model variant, ensuring real-time performance across different deployment scenarios.

% Concretely, domain-specific features $F_d$ (where $d=0$ represents the source domain and $d=1$ represents the target domain) are input to a discriminator $D$, which predicts the domain of these features. The discriminator is trained using cross-entropy loss, formulated as:

% which promotes feature alignment across domains by minimizing the discrepancy in domain-specific representations.

% with the goal of the network to fool this discriminator and produce domain-invariant representations.

% Adversarial Training (AT)-based UDA aims to learn domain-invariant representations by training a discriminator to predict the domain of input data based on detector features, while simultaneously optimizing features to mislead the discriminator. This approach is typically class-agnostic, focusing on domain-level alignment rather than class-specific feature distinctions. 

% will permit coarse-grained representations.

 % The proposed domain adaptation procedure for the generalized YOLO architecture is designed to operate across each detection scale—small (S), medium (M), and large (L)—leveraging labeled source data and unlabeled target data. The method ensures alignment at multiple levels of feature granularity, aligning high-level image features using $\img$ and fine-grained terrain features using $\inst$.

% To formalize this approach, a feature map $F$ is categorized as either global ($F^{G}$) or instance-level ($F^{I}$), and is further distinguished between source domain data ($F^{}_{S}$) and target domain data ($F^{}_{T}$), where $S \equiv (d=0)$ and $T \equiv (d=1)$. 
% This distinction enables tailored adaptation strategies for different feature representations.

% Detection heads in one-stage networks act as regressors for bounding box properties, class labels, and confidence scores. These detection heads produce outputs $D_*$, which correspond to spatial tensors with shape $\in C \times H \times W$, representing the detection confidence maps for each class and location. 

% Abstracting the design of the architecture in this manner allows for the integration of UDA components that remain agnostic to specific YOLO versions, as well as other classes of one-stage detectors such as EfficientDet~\cite{efficientdet} (although the evaluation of such detectors is out of the scope of this work). 

% PC minimizes the distance between source/target data distributions directly before detections are regressed, penalizing differences in finer features more heavily based on the assumption of celestial surface characteristics (e.g., scale, structure, etc). This direct alignment is insufficient on its own towards producing domain invariant features, however, given the difficulty of minimizing differences between unknown data distributions \textit{a priori}. Additional alignment through VSA is essential for enabling domain invariancy.

% To further bolster the effectiveness of UDA, we introduce additional mechanisms for instance alignment based on VSA clustering across two distinct datatypes, namely extracted detection \textit{instances} and pre-extraction \textit{features}.

% two categories of techniques, consisting of \textit{instance}

% \red{$\PC$ attempts to firstly regulates the instance features across scales in a direct manner and attempts to reduce the data distribution distance directly. Such a brute mechanism of alignment is insufficient on its own, however. As such, we study two further mechanisms for inducing instance-level alignment based on VSA clustering that can aid the domain-invariant representation generation. We propose to study two distinct clustering operations, one on extracted instances and one on the features directly.}

% with the expectation that scales with higher perceptive fields should contribute the most to alignment compared with smaller receptive fields (e.g., lower dimensional and higher abstracted features).

% without extracting them directly from multiple disjoint discriminator networks, a process by which we denote Perceptual Consistency (PC) The PC loss $\pc$ is computed as:

% Aside from $\pc$ which firstly regulates the instance features across scales in a general manner and attempts to reduce the data distribution distance directly. We further introduce two schemes for instance-specific comparisons: the first on the instances themselves (\textit{Instance Only}) and the second using detection activations yielded from the output features from the neck (\textit{Full Feature}).

% \textbf{Adversarial Training:}
% ~\autoref{fig:arch_inst_inst}

% \red{ViSGA VSA with region proposal network. one-stage don't have that. We begin our instance clustering by first extracting regions of interest (the detections). This increases the computation needed for training but does not take place during inference. After ROI extraction, we cluster instance embeddings through hierarchical clustering and employ adversarial training over mean cluster embeddings/representatives. In this scheme, the goal of instance discrimination is to then ensure domain-invariant features over detected terrain. Additionally, adversarial training can be forgone and we can learn instance alignment contrastively.}
Each cluster of embeddings is pooled to produce group-wise representatives, 

Upon convergence of the clustering process, embeddings within each cluster are pooled to generate an average representative embedding $Z_{c_i}$:
\begin{equation}
    Z_{c_i} = \frac{\sum_{i=0}^{N_{c_i}} z_i}{N_{c_i}}
\end{equation}
where $N_{c_i}$ is the number of embeddings assigned to the cluster $c_i$. Adversarial learning is applied to discriminate source/target instance embeddings in a similar fashion to~\autoref{eq:adv}.

% This approach provides flexibility by dynamically adjusting the number of cluster centers during the training, as opposed to fixing the cluster count as in techniques such as K-Means. 

% The mean cluster embeddings are then adversarial learned for domain discrimination in the same manner as described in~\autoref{sec:global_align}.


% \begin{equation}
%     \text{MaxLink}(A,B) = max\{dist(a,b): a \in A, b \in B\}
% \end{equation}
% where $A$ and $B$ denote the set of instance embeddings in each cluster, and $\text{dist}$ represents a vector distance measure such as cosine or Euclidean distance. A cluster radius parameter $\tau$ is defined 

% Initially, each instance is considered an independent cluster. At each iteration, the two clusters with the highest similarity are merged according to the cosine distance metric, given by:
% \begin{equation}
    % distance(z_i, z_j) = 1 - \frac{zi,zj}{||z_i||\cdot||z_j||}
% \end{equation}
% where $z_i$ and $z_j$ are the two instance embeddings. Using cosine similarity allows the pairing of instances that are spatially distant but visually similar. The merging process halts when the dissimilarity within a cluster, determined by a linkage function, surpasses a predefined cluster radius parameter $\tau$. To ensure cluster compactness, the complete-linkage heuristic is applied, maintaining the farthest distance between any two cluster members below $\tau$:

% \textit{Instance Clustering} in which we introduce a novel mechanism for improvement, \textit{Feature Clustering} introduced in YOCOv1, 

% as well as describing alternatives.

% as the overarching alignment mechanism within two categories of technique: \textit{Instance} and \textit{Feature} clustering. 

% we propose three novel techniques expanded from ideas in VSA, where the first is a general-purpose improvement and the latter two are interchangeable. These are a regularization scheme (Perceptual Consistency) and two techniques for VSA clustering (Instance and Feature). We start by defining our Perceptual Consistency regularization common to both VSA methods in~\autoref{sec:pc}, followed by each technique for VSA clustering (instance in~\autoref{sec:inst_clust} and feature in~\autoref{sec:feat_clust}).

% In total, we thoroughly study two categories of techniques for local alignment inspired by visual similarity-based clustering over instances and features, and introduce improvements in each. We start by describing the components common to each category, and then follow with descriptions and definitions of each category.

% Our method starts with PC loss, followed by two differing classes of techniques for instance alignment, dubbed Instance Only and Full Feature.

% We hypothesize that such a fine-grained means of feature comparison can constrain the domain gap ease the overall UDA difficulty on challenging space data, in particular high altitude imagery that exhibits overly-smoothed and less textured feature spaces where high-level feature discrimination may prove ineffective. 

% PC is essentially a weighted L1 loss between source and target pre-regression features.

% The core concept is to minimize the distance between like features and maximize the distance between unlike features across the domains. 

% When matching a single feature vector $F_{d}^{i}$ per class $i$ in each domain $d \in (0, 1)$, the max-margin contrastive loss is formulated as:
% \begin{align}
% \begin{split}
%     \mathcal{L}_{\text{Con}} &= \sum_{i}^{C} \left[ ||F_{0}^{i} - F_{1}^{i}||_2^2 \right. \\
%     &+ \sum_{j, j \neq i}^{C} \left. max\{0, m-||F_{0}^{i} - F_{1}^{j}||_2^2\} \right]
% \end{split}
% \end{align}
% \begin{equation}
%     \mathcal{L}_{\text{Con}} = \sum_{i}^{C} \left[ ||F_{0}^{i} - F_{1}^{i}||_2^2 + \sum_{j, j \neq i}^{C} max\{0, m-||F_{0}^{i} - F_{1}^{j}||_2^2\} \right]
% \end{equation}

% Where $C$ represents the number of classes and $m$ is the margin. Since the target data is unlabeled, the detector’s class predictions serve as pseudo-labels, as described in [??], allowing the application of Equation (??). In our analysis, we also explore the impact of disregarding class information. 





% \red{Above scheme is effectively ViSGA VSA ported to one-stage detection. As alluded to earlier, remote sensing of celestial surfaces at varying altitudes gives way to challenging visual spaces that prove difficult for VSA. During such observations, we hypothesize that not all/few features are actually/particularly effective in making the regressed detection. As such, we introduce a individual feature selection stage before inducing instance clustering. We refer to this process as Strong Feature Filtering (SFF). SFF works by....}

% we propose to methodically select or \textit{filter} the instance-level features before embeddings are garnered, effectively focusing only on \textit{strong} features and robust characteristics of each detection. 

% before continuing with subsequent instance embedding extraction, clustering, and adversarial/contrastive learning. 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/sff.pdf}
%     \caption{Strong Feature Filtering (SFF) module for distinct and robust feature selection. SFF ensures only object-relevant features are considered during instance alignment.}
%     \label{fig:sff}
% \end{figure}




% employing a channel-wise attention module over pre-extracted instance-level features $F^I_*$ in order to rank each channel (i.e., each individual feature)

% to assign each individual feature map ($F \in \mathbb{R}^{1\times H \times W}$) a score. 

% which scores each feature (i.e., ranks each channel). We then sort the resulting feature map and perform a Top-K selection before inducing instance embedding extraction and subsequent clustering.

% \red{During the instance extraction and clustering procedures, either adversarial or contrastive, as VSA procedures, the performance is completely dependent on the distinguishability of instance embeddings. 

% We hypothesize that in the presence of challenging space data, this might be difficult with many similarities and such. To alleviate this difficulty, we further propose to methodically select or \textit{filter} the features before embeddings are garnered, effectively focusing only on \textit{strong} features and characteristics that make for easy distinguishability and better clustering. 

% We begin by employing a channel-wise attention module over the pre-extracted instance features $F^I_*$ that scores each individual feature (i.e., ranks each channel). We then sort the resulting feature map and perform a Top-K selection before inducing instance embedding extraction and subsequent clustering. }

% \red{Explore alternative means for intra-feature clustering. YOCOv1 motivation sound, but had clear problems. K-Means with PC, or learn to pixel-pool directly with PC}

% where individual components of the pre-detection feature map were found to include many indistinguishable and ''non-object`` areas that led to ambiguity in the clustering, resulting in unstructured groups and weakly domain-invariant representations. 
% For this reason, we further examine two additional techniques at intra-feature

% It was further hypothesized that clustering full features in this manner would ease the UDA task for space images where the presence of many object classes are similar, by exploiting the residual areas in the feature map around detections instead of solely focusing on the detections themselves.

% The loss configurations for $\inst$ based on activation clustering differ from ROI-based $\inst$ (\autoref{fig:inst-advcont}) by grouping the set of source and target object-level features into various clusters. 

% YOCOv1 showed however to be 

% Similar to SFF, for the adversarial case we directly pool pixels based on channel attention activation scoring instead of clustering to yield a final feature map of size 1xhxw. Our attention pooling mechanism is similar to PTAP~\cite{ptap}, based on the priority of activations, defined as follows. To compute the priority, we first apply a channel attention module~\cite{??} to assign importance weights to each channel of the feature map. Specifically, we perform global average pooling (GAP)~\cite{??}, followed by a 1D convolution and a sigmoid function, sequentially, on the feature map $F_x \in \mathbb{R}^{C \times H \times W}$. The weighted feature map $F_w$ is broadcast spatially to yield Strong Pixel Pooling (SPP) procedure:

% \subsection{Learning Objectives}
% Contrastive and adversarial region-of-interest (ROI) loss configurations for $\inst$ offer complementary approaches for improving feature alignment and discrimination in object detection. Detected regions are first extracted from features through ROI extraction. These regions are then processed using one of two methods: contrastive learning ($\con$), which directly optimizes similarity between region embeddings, or adversarial training ($\adv$), which employs discriminators on mean cluster embeddings to enhance domain invariance. To maintain consistency, a perceptual loss
% ($\pc$) enforces alignment between features prior to detection. Additionally, a learnable Top-K selection filter highlights the most impactful features, focusing the model’s attention on the most relevant information for improved performance.

% This ultimately drives the feature extraction into producing domain-invariant representations that are performant in each domain. 

To ensure that the features from the two domains become indistinguishable by the discriminator, the loss in~\autoref{eq:adv} must be maximized with respect to the features $F_d$. This objective is achieved by introducing a Gradient Reverse Layer (GRL)~\cite{grl}, positioned at the first layer of the discriminator network. The GRL applies a negative scaling factor to the gradients during backpropagation, effectively reversing the gradient flow. This mechanism ensures that while the discriminator is trained to minimize the cross-entropy loss for domain classification, the feature extractor is optimized to maximize the same loss. 

==> sections/_notes_relwork.tex <==
\begin{itemize}
    \item VSA is a concept for UDA proposed by ViSGA~\cite{visga}
    \item It argues that visual similarities in the feature space are a great anchor to bridge the domain distribution gap
    \item ViSGA~\cite{visga} introduced VSA for two-stage faster rCNN. Recently, VSA has been improved:
    
    \item MLFA: Toward Realistic Test Time Adaptive Object Detection by Multi-Level Feature Alignment~\cite{vsa_two2}. Test Time Adaptive Object Detection (TTA-OD) is a novel approach enabling detectors to adapt and predict in real-time during testing, addressing limitations in existing unsupervised domain adaptation methods. Essential for tasks like self-driving, TTA-OD is enhanced by our multi-level feature alignment (MLFA) method, which uses streaming target domain data to adapt models online. MLFA aligns features by: (i) performing global alignment to extract domain-invariant features and (ii) using cluster alignment to match category-specific features across domains. This alignment enables detectors to capture both domain-invariant and category-specific features for improved adaptability across environments.
    
    \item Improving Object Detection via Local-global Contrastive Learning~\cite{vsa_two3}. Visual domain gaps challenge object detection, and while image-to-image translation can help, current methods falter in complex scenes due to reliance on costly annotations. We propose a new image-to-image translation method for cross-domain detection, using a contrastive learning framework with spatial attention to distinguish objects from background without explicit annotations. By contrasting local and global information, our approach enables high detection performance under domain shifts, achieving state-of-the-art results across three challenging benchmarks without model fine-tuning.
    
    \item JFDI: Joint Feature Differentiation and Interaction for domain adaptive object detection~\cite{vsa_two6}. However, prior methods mainly focused on aligning domain-invariant features and overlooked target-specific features. To address this, we propose Joint Feature Differentiation and Interaction (JFDI), a novel feature learning method that enhances detector adaptability. JFDI uses a dual-path architecture: one path aligns domain-invariant features with source data using multiple discriminators, while the other learns target-specific features from pseudo-labeled target data. An interactive mechanism between these paths ensures stable feature learning and reduces pseudo-label noise. We also introduce a hierarchical pseudo-label fusion module for more reliable results. Theoretical analysis of JFDI’s generalization error bound supports its effectiveness.
    
    \item Cross Domain Object Detection via Multi-Granularity Confidence Alignment based Mean Teacher~\cite{vsa_two9}. While Mean Teacher has shown promise, pseudo labeling remains a bottleneck in mutual learning. This study identifies confidence misalignment—including overconfidence at the category level, inconsistency at the instance level, and misfocusing at the image level—as a source of noisy pseudo labels that degrade target domain performance. To address this, we introduce Multi-Granularity Confidence Alignment Mean Teacher (MGCAMT), a framework for cross-domain object detection that simultaneously aligns confidence across category, instance, and image levels to improve pseudo supervision. MGCAMT includes: (i) Classification Confidence Alignment (CCA), which models category uncertainty using Evidential Deep Learning (EDL) to filter out incorrect labels; (ii) Task Confidence Alignment (TCA), which enhances task interaction to align classification and localization; and (iii) Focusing Confidence Alignment (FCA), which uses Mean Teacher outputs for supervised learning without label assignment to focus on holistic target domain information. These procedures work synergistically, improving performance through cooperative learning. For one and two-stage detectors.
    
    \item D-MASTER: Mask Annealed Transformer for Unsupervised Domain Adaptation in Breast Cancer Detection from Mammograms~\cite{vsa_transformer1}. Recent advancements in masked image modeling have proven effective for unsupervised domain adaptation (UDA), but face challenges in cross-domain breast cancer detection due to the smaller size of regions of interest compared to natural images. This often leads to higher false positives and noisy pseudo-labels. To address these issues, we propose D-MASTER, a transformer-based Domain-invariant Mask Annealed Student Teacher autoencoder. D-MASTER adaptively masks and reconstructs multi-scale feature maps to capture reliable target domain features, and incorporates adaptive confidence refinement to filter pseudo-labels, ensuring high-quality detections. We also introduce the RSNA-BSD1K, a subset of 1000 bounding box-annotated mammograms from the RSNA Breast Screening Dataset, to support further BCDM research.
    
    \item REACT: Remainder Adaptive Compensation for Domain Adaptive Object Detection~\cite{vsa_two10}. Recent studies use a shared feature extractor across source and target domains to capture domain-invariant features and task-relevant information, relying on feature-alignment constraints and source annotations. However, this approach discards some task-relevant information from the target domain due to domain gaps and lack of target annotations, compromising target domain discrimination. To address this, we propose the REACT (REmainder Adaptive CompensaTion) network, which adaptively compensates for discarded features by incorporating remainder features that contain valuable task-relevant information. REACT introduces a remainder branch to recover these features and adaptively use them to enhance target domain discrimination. Faster R-CNN.

    \item ==============================
    
    \item Most existing unsupervised domain adaptive object detection methods rely on two-stage detectors like Faster-RCNN, as the region proposal network (RPN) helps achieve instance-level domain adaptation (SDAN-YOLO Abstract). Lately, research in bringing VSA to one-stage detectors, which is attractive for in-situ space use bc two-stage models are too big and computationally expensive (although, may be a performance accuracy hit as two-stage generally more expressive than one-stage):
    
    \item OSSA: Unsupervised One-Shot Style Adaptation~\cite{vsa_yolo1}. Deep neural networks often struggle in out-of-distribution scenarios due to domain style differences between training and target data. To address this, we propose One-Shot Style Adaptation (OSSA), an unsupervised domain adaptation method that uses a single unlabeled target image to approximate the target domain style. OSSA perturbs the style statistics from the target image to generate diverse target styles, which are then applied to a labeled source dataset using Adaptive Instance Normalization (AdaIN). Experimental results show OSSA achieves state-of-the-art performance in one-shot domain adaptation, even outperforming methods using thousands of unlabeled target images. OSSA excels in weather, sim2real, and visual-to-thermal adaptations, demonstrating its effectiveness in bridging the style gap. Its simplicity and efficiency make it easy to integrate into existing frameworks, offering a practical solution for applications with limited data.
    
    \item Tri-Flow-YOLO: Counter helps to improve cross-domain object detection~\cite{vsa_yolo2}. Intelligent detection models have achieved significant success, but still face performance degradation and low accuracy in cross-domain scenarios. To address this, we propose the multi-supervised Tri-Flow-YOLO model to enhance object detection across varying scales in cross-domain conditions. Building on the fully-supervised YOLOv5 detection branch, we introduce two additional mutually supportive task branches. First, an unsupervised adversarial classification flow is added to achieve feature alignment and stabilize cross-domain performance. Second, a weakly-supervised object counting flow improves the model’s attention to all objects, boosting detection efficiency. Additionally, I-Mosaic and iCIOU are specifically designed for small, challenging objects, enriching positive samples and alleviating the imbalance between positive and negative samples in the anchor-based model.
    
    \item AdvMix: Adversarial Mixing Strategy for Unsupervised Domain Adaptive Object Detection~\cite{vsa_yolo3}. We propose a domain adaptive method, Adversarial Mixing (AdvMix), that jointly trains a label-rich source domain and an unlabeled target domain through adversarial feature alignment and a self-training strategy. To reduce the style gap, we introduce the Adversarial Gradient Reversal Layer (AdvGRL), which includes a global-level domain discriminator for feature alignment and an adversarial weight mapping function to enhance domain-invariant feature stability via hard example mining. To address the content gap, we implement a region mixing self-supervised strategy, where the most confident target image region is merged with the source image and self-supervised with consistency loss. We also propose a strict confidence metric that combines object and bounding box uncertainty to improve self-training reliability.
    
    \item Inter-Domain Invariant Cross-Domain Object Detection Using Style and Content Disentanglement for In-Vehicle Images~\cite{vsa_retinanet}. We introduce IDI-SCD, a novel method that simultaneously addresses both the style and content gaps in domain adaptation. The domain gap is first disentangled into the style and content gaps, generating corresponding intermediate domains. During training, we focus on one gap at a time to achieve inter-domain invariance—tackling the content gap while preserving the style gap and vice versa. A style-invariant loss reduces the style gap, while the mean teacher self-training framework addresses the content gap. Additionally, a multiscale fusion strategy is introduced to improve the quality of pseudo-labels, enhancing detection performance for extreme-scale objects. Extensive experiments on four mainstream in-vehicle image datasets demonstrate the effectiveness of our approach.
    
    \item Multi-vessel target tracking with camera fusion for unmanned surface vehicles~\cite{vsa_yolo4}. With the decreasing availability of sailors, the development of autonomous ships has gained increasing focus. A key area of research is automatic recognition systems that can replace human vision. Traditional sensors like RADAR and AIS have limitations such as blind spots and restricted range. To address this, we propose a recognition method utilizing multiple cameras—electro-optical and infrared radiation cameras—alongside traditional sensors for accurate maritime obstacle detection and dynamic motion estimation. Deep-learning models trained on real-sea images detect obstacles, and an adaptive tracking filter is used for motion estimation. Additionally, fusion of tracked data from multiple cameras compensates for individual sensor limitations, enhancing tracking results. Field tests with Unmanned Surface Vehicles (USVs) show that the method successfully converges tracking within GPS error ranges, with significantly improved results through multi-camera data fusion.
    
    \item SDAN-YOLO: Self-attention domain adaptive network for YOLOv7~\cite{vsa_yolo5}.  However, these methods struggle with real-time performance, which is crucial in applications like autonomous driving. To address this, we propose a self-attention domain adaptive network for the one-stage YOLOv7 detector. This network uses self-attention to extract foreground position information, acting as an RPN for instance-level adaptation. We also introduce local self-attention augmentation to reduce attention noise, ensuring accurate focus on foreground targets. Additionally, we apply coarse-to-fine alignment: global domain adaptation initially aligns global features, followed by local adaptation for precise alignment of foreground features.
    
    \item Misalignment-resistant domain adaptive learning for one-stage object detection~\cite{vsa_one_stage_general}. DA on one stage suffers from two experimentally identified limitations: foreground misalignment and localization misalignment. the "Mask-Based Domain Discriminator" functions primarily as a thresholding mechanism that differentiates foreground from background based on mean and standard deviation, while the "Localization Discriminator" aligns bounding boxes across branches by relying on the height-to-width ratio as a standard localization-invariant feature in cross-domain detection tasks for general-purpose one-stage detectors.

    \item Degradation Type-Aware Image Restoration for Effective Object Detection in Adverse Weather~\cite{vsa_yolo6}. While CNN-based object detection has advanced, adverse weather disrupts sensor clarity, reducing detection accuracy. Conventional methods address this with image restoration tailored to specific conditions, limiting adaptability across weather types. To address this, we propose DTRDNet, a degradation-aware, restoration-assisted detection network with a shared feature encoder (SFE), a degradation-sensitive image restoration decoder (DDIR), and a degradation category predictor (DCP). During training on a mixed weather dataset, DDIR leverages degradation type data to prevent interference with clean images, while DCP enhances SFE’s adaptability to various weather. For real-time inference, DCP and DDIR can be omitted as needed. 

    \item Cross-pollination of knowledge for object detection in domain adaptation for industrial automation~\cite{vsa_yolo7}. This study introduces a Cross-Pollination of Knowledge (CPK) strategy, inspired by botanical processes, for domain adaptation. CPK merges selected target and source samples at input to improve OD results by aligning features effectively. Additionally, we introduce the Planeat digit recognition dataset of 231 images, using a self-supervised Domain Adaptation (UDA) method that trains on both domains unsupervised, identifying and augmenting high-confidence target regions.

    \item Degradation Modeling for Restoration-enhanced Object Detection in Adverse Weather Scenes~\cite{vsa_one_stage_general2}. Mainstream methods often overlook object detection in degraded images, limiting their effectiveness in adverse weather conditions. We propose RDMNet, a Restoration-enhanced object detection network with Degradation Modeling. RDMNet features a dual-branch architecture that integrates restoration into the detection process to capture more information from degraded images. To enhance adaptability across weather types, we model multi-scale degradation representations to guide feature transformation in both branches. A multi-scale bi-directional feature fusion block enables cross-task integration, and a restoration weight decay strategy further optimizes training.

    \item Self-Supervised Domain Adaptation for 6DoF Pose Estimation~\cite{vsa_one_stage_general3}. To address this, we propose domain adaptation for self-supervised 6DoF pose estimation, introducing an effective approach to reduce domain discrepancy. Our method incorporates a multi-level domain adaptation module, operating at both the image and instance levels, to learn domain-invariant features. We also apply entropy-based alignment to minimize representation embedding entropy.
\end{itemize}







Unsupervised Domain Adaptation (UDA) has become a prominent technique for training object detectors on datasets that differ significantly from those encountered in operational environments, particularly when labeled target domain data is scarce or unavailable. By leveraging unlabeled data from the target domain, UDA allows for the adaptation of models trained on source domain data, bridging the domain gap. One of the most widely used approaches in UDA for object detection is Visual Similarity-based Alignment (VSA~\cite{visga}), originally proposed for the two-stage network Faster R-CNN. VSA aims to align feature distributions between the source and target domains by focusing on visual similarities of region proposals, enabling the transfer of learned knowledge from the source domain to the target domain without requiring explicit labels for the target data. This approach is seen as a cost-effective and efficient way to exploit existing object detection pipelines for domain adaptation. Over time, numerous novel techniques have been introduced to enhance the effectiveness of VSA. Test Time Adaptive Object Detection (TTA-OD) tackles real-time adaptation challenges by introducing Multi-Level Feature Alignment (MLFA), which aligns global domain-invariant features and category-specific features using streaming target domain data, thus enabling models to adapt during testing~\cite{vsa_two2}. Similarly, contrastive learning techniques have been employed to address visual domain gaps in object detection. A notable approach uses spatial attention in an image-to-image translation framework, distinguishing objects from the background through local-global contrastive learning without requiring explicit annotations, achieving state-of-the-art performance across multiple benchmarks~\cite{vsa_two3}. Further, Joint Feature Differentiation and Interaction (JFDI) enhances detector adaptability by using a dual-path architecture. One path aligns domain-invariant features using discriminators, while the other learns target-specific features from pseudo-labeled data. An interactive mechanism between these paths ensures stable learning and reduces noise in pseudo-labels~\cite{vsa_two6}.

In addition, methods focused on improving pseudo-label quality have also emerged. Multi-Granularity Confidence Alignment Mean Teacher (MGCAMT) addresses confidence misalignment in pseudo-labeling by aligning confidence at category, instance, and image levels. This multi-tier approach, which includes Classification Confidence Alignment (CCA), Task Confidence Alignment (TCA), and Focusing Confidence Alignment (FCA), enhances performance through cooperative learning and applies to both one- and two-stage detectors~\cite{vsa_two9}. In the context of breast cancer detection, D-MASTER leverages masked image modeling for unsupervised domain adaptation (UDA), adaptively masking and reconstructing multi-scale feature maps to capture reliable target domain features. It also integrates adaptive confidence refinement to filter out noisy pseudo-labels, ensuring high-quality detections~\cite{vsa_transformer1}. Lastly, the REACT network addresses domain gaps in feature extraction by compensating for discarded task-relevant features through a remainder branch, which enhances target domain discrimination and improves the adaptation process in Faster R-CNN~\cite{vsa_two10}. These methods collectively enhance the reliability and adaptability of object detection models across challenging domain shifts.

Although VSA is a performant means for UDA in two-stage detectors, VSA applied to one-stage detection (which is more computationally efficient) is more difficult due to the lack of a distinct region proposal network. OSSA (Unsupervised One-Shot Style Adaptation)~\cite{vsa_yolo1}, tackles domain style differences by using a single unlabeled target image to approximate the target domain style, applying adaptive instance normalization (AdaIN) to adapt a labeled source dataset. Tri-Flow-YOLO~\cite{vsa_yolo2} enhances cross-domain object detection by introducing additional task branches for unsupervised adversarial classification and weakly-supervised object counting, improving feature alignment and attention to small objects. AdvMix~\cite{vsa_yolo3} takes a different approach with adversarial feature alignment and self-training, employing adversarial gradient reversal layers and region mixing strategies to reduce style and content gaps. Methods such as IDI-SCD~\cite{vsa_retinanet} also explore disentangling style and content gaps, using a style-invariant loss and a mean teacher framework for content alignment.

For real-time applications, particularly in autonomous driving, domain adaptation methods that focus on one-stage detectors have shown great promise. SDAN-YOLO~\cite{vsa_yolo5} proposes a self-attention mechanism to extract foreground position information for instance-level adaptation in YOLOv7, combining global and local domain adaptation techniques. However, challenges such as foreground misalignment and localization misalignment persist in one-stage detectors. The Mask-Based Domain Discriminator and Localization Discriminator proposed in one method~\cite{vsa_one_stage_general} address these issues by focusing on foreground-background differentiation and bounding box alignment, respectively. Similarly, Degradation Type-Aware Image Restoration methods like DTRDNet~\cite{vsa_yolo6} integrate weather degradation restoration into the detection process, improving robustness in adverse conditions.

Other methods focus on cross-domain knowledge sharing, such as the Cross-Pollination of Knowledge (CPK) strategy~\cite{vsa_yolo7}, which merges target and source samples at the input level for better feature alignment. Meanwhile, RDMNet~\cite{vsa_one_stage_general2} introduces restoration-enhanced object detection, incorporating degradation modeling to improve detection in degraded images caused by adverse weather. Lastly, Self-Supervised Domain Adaptation for 6DoF Pose Estimation~\cite{vsa_one_stage_general3} provides a novel solution for reducing domain discrepancy in pose estimation through a multi-level domain adaptation module that operates at both image and instance levels. These advancements demonstrate the increasing efficiency and adaptability of one-stage domain adaptation techniques for various real-world scenarios.















Although Visual Similarity-based Alignment (VSA) has proven effective for Unsupervised Domain Adaptation (UDA) in two-stage detectors, its application to one-stage detectors is more challenging due to the absence of a distinct region proposal network. To address this, approaches like Unsupervised One-Shot Style Adaptation (OSSA~\cite{vsa_yolo1}) use a single unlabeled target image to approximate the target domain style, applying adaptive instance normalization (AdaIN) to adapt a labeled source dataset. Other methods, such as AdvMix~\cite{vsa_yolo3}, employ adversarial feature alignment combined with self-training strategies, utilizing adversarial gradient reversal layers and region mixing to address style and content gaps. Tri-Flow-YOLO~\cite{vsa_yolo2} improves cross-domain object detection by adding unsupervised adversarial classification and weakly-supervised object counting branches, which enhance feature alignment and detection of small objects. Additionally, methods like IDI-SCD~\cite{vsa_retinanet} focus on disentangling style and content gaps, using style-invariant loss and a mean teacher framework for content alignment.

For real-time applications such as autonomous driving, one-stage domain adaptation methods have gained traction due to their computational efficiency. SDAN-YOLO~\cite{vsa_yolo5} introduces a self-attention mechanism to extract foreground position information for instance-level adaptation, combining global and local domain adaptation techniques. However, challenges such as foreground misalignment and localization misalignment persist. The Mask-Based Domain Discriminator and Localization Discriminator~\cite{vsa_one_stage_general} address these by differentiating foreground from background and aligning bounding boxes, respectively. Degradation Type-Aware Image Restoration methods, such as DTRDNet~\cite{vsa_yolo6}, further enhance robustness by integrating weather degradation restoration into the detection process. Cross-domain knowledge sharing techniques, like the Cross-Pollination of Knowledge (CPK) strategy~\cite{vsa_yolo7}, improve feature alignment by merging target and source samples at the input level. Additionally, RDMNet~\cite{vsa_one_stage_general2} incorporates restoration-enhanced object detection with degradation modeling, improving performance in degraded conditions. Lastly, Self-Supervised Domain Adaptation for 6DoF Pose Estimation~\cite{vsa_one_stage_general3} reduces domain discrepancy in pose estimation through a multi-level domain adaptation module that operates at both the image and instance levels. These advancements highlight the growing efficiency and adaptability of one-stage domain adaptation methods for a variety of real-world scenarios.

% ==================== PAR1
Celestial terrain detection has historically focused on lunar craters with image processing methods, where deep learning has only recently been explored. Convolutional Neural Networks (CNNs) have been used for the classification of craters found with edge detection techniques~\cite{cda1} or through cascaded networks with synthetic data~\cite{cda9}. Semantic segmentation of craters and crater rims has found popularity with U-Net architectures~\cite{cda2,cda3,cda4} that are trained on Digital Elevation Maps (DEMs)~\cite{cda2} and infrared response maps~\cite{cda3,cda4}. Methodical fusion of CNNs, image processing, and DEM data has been additionally successful~\cite{cda8,cda10}. Object detection algorithms were first employed for crater detection with YOLOv3~\cite{cda5}, Faster R-CNN~\cite{cda6}, and Mask R-CNN~\cite{cda7} architectures using highly curated and post-processed datasets of prior mission data. There has been less attention paid to detecting general multi-class terrain features from nadir-facing orbital platforms, with the only such works performing density analysis over traditional hand-crafted feature points (e.g., SIFT~\cite{sift}) for hazard labeling~\cite{terrain1} and ensemble-network learning with multiple Faster R-CNNs~\cite{terrain3}. To date, the only method exploring UDA for general-purpose terrain detection was \textit{You Only Crash Once} (YOCOv1~\cite{yoco}), which studied the singular VSA procedure of intra-feature clustering within the non-real-time YOLOv3 architecture. 

Prior approaches encounter significant challenges in practical onboard execution. Traditional image processing algorithms are computationally expensive unless specifically optimized through mission-specific acceleration techniques~\cite{mht, profiling}. Similarly, object detection models such as YOLOv3 and Faster R-CNN cannot achieve real-time or near-real-time performance when deployed onboard current spacecraft hardware~\cite{profiling}. Additionally, there are substantial difficulties in training these learning-based methods. For example, the use of synthetic training data drastically degrades operational performance due to domain shift, while the application of domain adaptation in space applications has remained under-explored. Furthermore, earlier methods have largely focused on crater detection and fail to generalize to other prominent terrain features—such as dunes, mountains, and ridges—that may be more common on extraterrestrial bodies. In these multi-class scenarios, creating training datasets from DEMs becomes even more complex. 
The reliance on DEMs or extensive post-processing, including the hand-labeling of imagery from previous missions, is both resource-intensive and non-transferable to novel, unexplored environments; a critical limitation to future space missions that require terrain detection on previously unexplored worlds such as Titan~\cite{titan} and Enceladus~\cite{enceladus}.

% ==================== PAR2
VSA was originally proposed within two-stage frameworks that employ disparate networks for object region proposals~\cite{visga}, where these proposals from source and target domains are aligned by visual similarity clustering as opposed to class or pseudo-class labels. Over time, numerous techniques have been introduced to enhance the effectiveness of VSA. An online algorithm is proposed in~\cite{vsa_two2} which clusters instance-level detections after global domain-invariant feature extraction. Image-to-image translation with clustering and contrastive learning has been employed to generate intermediate style-consistent data~\cite{vsa_two3}, while the grounding of pseudo-labels has found popularity in both domain-invariant feature learning~\cite{vsa_two6} and mean teacher-student frameworks~\cite{vsa_two9}. The use of transformers has found popularity in~\cite{vsa_transformer1}, while additional heads that compensate for discarded task-relevant features bolstered performance in~\cite{vsa_two10}.

The adoption of VSA into one-stage detectors has been traditionally challenging, inherently due to the absence of region proposals. Methods like OSSA~\cite{vsa_yolo1} use a single unlabeled target image with AdaIN to adapt the source dataset, while AdvMix~\cite{vsa_yolo3} combines adversarial feature alignment and self-training to address style and content gaps. Tri-Flow-YOLO~\cite{vsa_yolo2} enhances detection by adding adversarial and weakly-supervised branches, and IDI-SCD~\cite{vsa_retinanet} disentangles content gaps through a style-invariant loss. In real-time applications like autonomous driving, SDAN-YOLO~\cite{vsa_yolo5} introduces self-attention for instance-level adaptation, while addressing misalignment issues with mask-based and localization discriminators~\cite{vsa_one_stage_general}. Methods like DTRDNet~\cite{vsa_yolo6} improve robustness in adverse conditions through weather degradation restoration, and CPK~\cite{vsa_yolo7} enhances feature alignment by merging target and source samples. RDMNet~\cite{vsa_one_stage_general2} integrates restoration and degradation modeling for improved detection in degraded conditions, and Self-Supervised Domain Adaptation for 6DoF Pose Estimation~\cite{vsa_one_stage_general3} reduces domain discrepancy through a multi-level adaptation module.

% aligning the feature distributions 

% Unsupervised Domain Adaptation (UDA) has become a prominent technique for training object detectors on datasets that differ significantly from those encountered in operational environments, particularly when labeled target domain data is scarce or unavailable. One of the most widely used approaches in UDA for object detection is Visual Similarity-based Alignment (VSA~\cite{visga}), originally proposed for two-stage networks with disparate region proposal networks. 

% VSA aims to align feature distributions between the source and target domains by focusing on visual similarities of the proposals, enabling the transfer of learned knowledge from the source domain to the target domain without requiring explicit labels or pseudo-labels. 

% OSSA~\cite{vsa_yolo1} leverages a single unlabeled target image, while AdvMix~\cite{vsa_yolo3} combines adversarial alignment and self-training to bridge style gaps. 

% Tri-Flow-YOLO~\cite{vsa_yolo2} incorporates adversarial and weakly-supervised branches, and IDI-SCD~\cite{vsa_retinanet} introduces a style-invariant loss. For real-time applications like autonomous driving, SDAN-YOLO~\cite{vsa_yolo5} utilizes self-attention for instance-level adaptation and addresses misalignments with mask-based and localization discriminators~\cite{vsa_one_stage_general}. Robustness in adverse conditions is improved by methods like DTRDNet, which integrates weather degradation restoration~\cite{vsa_yolo6}, and RDMNet, which performs degradation modeling~\cite{vsa_one_stage_general2}. Additionally, CPK~\cite{vsa_yolo7} merges target and source samples for better feature alignment, while self-supervised domain adaptation methods reduce domain discrepancies through multi-level adaptation~\cite{vsa_one_stage_general3}.



% ============================ PAR3
Images of celestial terrain present unique challenges due to homogeneous regions, smoothness, and the absence of distinct gradient or texture variations, particularly at higher altitudes. These properties can complicate traditional object detection pipelines, let alone in the presence of data domain gap. VSA is a promising direction to alleviate such challenging scenes by promoting network correlations in global terrain feature structure, appearance, shape, and distinction to the uniform background surface, although VSA studies in this context are relatively non-existent. Earth-based aerial VSA was previously studied~\cite{vsa_aerial1}, although without a focus on geological terrain. YOCOv1~\cite{yoco} is the only such work that targets a form of generalizable multi-class celestial terrain detection in UDA settings by employing VSA. YOCOv1 introduces the concept of intra-feature clustering to solve the celestial appearance challenge, drawing correlations between the activations that garner detections and minimizing the domain shift in how these activations appear. This is in stark contrast to earlier methods that extract object features before any clustering operation, forgoing any additional background features. This proved useful in single-class feature-full scenes (such as terrestrial urban driving) but saw performance degradations in multi-class celestial surfaces (like Mars) where features such as craters, dunes, and mountains were hard to distinguish by activation discernability alone. Additionally, the practicality of YOCOv1 is questioned as the YOLOv3 architecture in which is it based is unable to execute in real-time on spacecraft hardware~\cite{profiling}.


% by employing VSA with synthetic training data. Unlike other methods that perform instance-level alignment using extracted regions of detection, YOCOv1 performs VSA by clustering and aligning intermediate feature maps, drawing correlations between the activations that garner detections and minimizing the domain shift in how these activations appear. 

==> sections/discussion.tex <==
\section{Discussion and Limitations}\label{sec:discussion}

==> sections/problem.tex <==
\section{Problem Formulation}\label{sec:problem}
\red{Paragraph on ViSGA two-stage approach with formulas}

\red{Pargraph on YOCOv1, adaptation of the ViSGA approach on hierarchical clustering individual channels of feature maps into similar groups}

\red{Towards a lightweight UDA technique for one-stage network that }

==> tables/map_12/map_asteroid.tex <==
\begin{table*}
\centering
\caption{Mean Average Precision (IOU=0.5) results (\%) for \textit{Asteroid}. Green and yellow indicate the highest and second-highest performing method for each YOLO model/size variant.}
\label{tab:map_asteroid}
\resizebox{\textwidth}{!}{%
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[1]Q[40]Q[50]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[50]},
  cells = {c},
  cell{1}{3} = {c=11}{},
  cell{2}{3} = {r=2}{},
  cell{2}{4} = {c=3}{},
  cell{2}{7} = {c=3}{},
  cell{2}{10} = {c=3}{},
  cell{2}{13} = {r=2}{},
  cell{4}{1} = {r=8}{},
  vline{3} = {4-11}{},
  vline{4,7,10,13} = {2-11}{dashed},
  hline{1} = {-}{},
  hline{3} = {4-12}{dashed},
  hline{4} = {3-13}{},
  hline{12} = {-}{},
}
 &  & \textbf{Method} &  &  &  &  &  &  &  &  &  & \\
 &  & {Source\\Only} & Adversarial &  &  & Contrastive &  &  & Full Feature &  &  & {Target\\Only}\\
 &  &  & ROI & Perceptual & Top-K & ROI & Perceptual & Top-K & YOCOv1 & K-Means & PTAP & \\
\begin{sideways}\textbf{Architecture}\end{sideways}

& 5-N & \phantom{0}5.4 & 10.9 & \SetCell[c=1]{c, olive9}\textbf{53.1} & 15.0 & 37.6 & 39.9 & 26.2 & 38.0 & 32.9 & \SetCell[c=1]{c, yellow9}\textbf{47.6} & 92.0\\
& 5-S & 35.5 & \SetCell[c=1]{c, yellow9}\textbf{56.5} & 44.7 & 34.9 & 37.2 & 52.8 & 31.8 & 50.2 & \SetCell[c=1]{c, olive9}\textbf{57.0} & 35.7 & 92.4\\
& 5-M & 32.8 & 51.2 & \SetCell[c=1]{c, yellow9}\textbf{61.0} & \phantom{0}4.6 & 44.2 & 40.4 & \SetCell[c=1]{c, olive9}\textbf{61.2} & 44.7 & 49.5 & 53.5 & 92.6\\
& 6-N & 66.3 & 58.8 & 65.5 & 60.1 & 58.8 & 63.2 & 61.8 & \SetCell[c=1]{c, yellow9}\textbf{67.3} & \SetCell[c=1]{c, olive9}\textbf{67.4} & 62.8 & 91.9\\
& 6-S & 64.3 & 58.9 & \SetCell[c=1]{c, olive9}\textbf{66.2} & \SetCell[c=1]{c, yellow9}\textbf{65.7} & 58.9 & 65.3 & 63.0 & 59.8 & 62.4 & 60.7 & 92.8\\
& 8-N & 26.0 & 31.1 & 43.4 & \SetCell[c=1]{c, olive9}\textbf{60.7} & 40.3 & 17.8 & \SetCell[c=1]{c, yellow9}\textbf{55.3} & 34.0 & 43.3 & 24.1 & 91.8\\
& 8-S & \SetCell[c=1]{c, yellow9}\textbf{55.3} & 36.8 & 55.2 & \SetCell[c=1]{c, olive9}\textbf{56.1} & 22.1 & 45.5 & 53.0 & \SetCell[c=1]{c, olive9}\textbf{56.1} & 13.2 & 18.7 & 92.5\\
& 8-M & 25.2 & 49.0 & 49.5 & \SetCell[c=1]{c, olive9}\textbf{53.8} & 41.9 & 45.8 & 41.2 & \SetCell[c=1]{c, yellow9}\textbf{52.3} & 32.6 & 40.0 & 93.2\\

\end{tblr}
}
\end{table*}

==> tables/map_12/map_mars.tex <==
\begin{table*}
\centering
\caption{Mean Average Precision (IOU=0.5) results (\%) for \textit{Mars}. Green and yellow indicate the highest and second-highest performing method for each YOLO model/size variant.}
\label{tab:map_mars}
\resizebox{\textwidth}{!}{%
\begin{tblr}{
  width = \linewidth,
  % Used to be 60s
  colspec = {Q[1]Q[40]Q[50]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[50]},
  cells = {c},
  cell{1}{3} = {c=11}{},
  cell{2}{3} = {r=2}{},
  cell{2}{4} = {c=3}{},
  cell{2}{7} = {c=3}{},
  cell{2}{10} = {c=3}{},
  cell{2}{13} = {r=2}{},
  cell{4}{1} = {r=8}{},
  vline{3} = {4-11}{},
  vline{4,7,10,13} = {2-11}{dashed},
  hline{1} = {-}{},
  hline{3} = {4-12}{dashed},
  hline{4} = {3-13}{},
  hline{12} = {-}{},
}
 &  & \textbf{Method} &  &  &  &  &  &  &  &  &  & \\
 &  & {Source\\Only} & Adversarial &  &  & Contrastive &  &  & Full Feature &  &  & {Target\\Only}\\
 &  &  & ROI & Perceptual & Top-K & ROI & Perceptual & Top-K & YOCOv1 & K-Means & PTAP & \\
\begin{sideways}\textbf{Architecture}\end{sideways}

& 5-N & 51.1 & 57.9 & 55.7 & \SetCell[c=1]{c, olive9}\textbf{62.4} & 56.4 & 53.6 & 52.2 & \SetCell[c=1]{c, yellow9}\textbf{59.3} & 54.3 & 58.4 & 93.7\\
& 5-S & 64.0 & \SetCell[c=1]{c, yellow9}\textbf{65.4} & 64.0 & 64.6 & 60.7 & 60.9 & \SetCell[c=1]{c, olive9}\textbf{66.3} & 62.7 & 55.5 & 63.2 & 94.2\\
& 5-M & 63.2 & 68.3 & \SetCell[c=1]{c, yellow9}\textbf{71.4} & 66.1 & \SetCell[c=1]{c, olive9}\textbf{71.6} & 65.9 & 68.4 & 68.8 & 65.4 & 62.9 & 94.9\\
& 6-N & \SetCell[c=1]{c, yellow9}\textbf{64.9} & 58.2 & 56.7 & 56.1 & 55.2 & 59.2 & 55.8 & \SetCell[c=1]{c, olive9}\textbf{65.0} & 60.4 & 50.8 & 93.9\\
& 6-S & 60.9 & 64.3 & 66.0 & 64.3 & 65.7 & \SetCell[c=1]{c, yellow9}\textbf{69.2} & \SetCell[c=1]{c, olive9}\textbf{69.6} & 65.5 & 66.2 & 64.2 & 94.3\\
& 8-N & 57.4 & 51.9 & 55.9 & 51.7 & \SetCell[c=1]{c, yellow9}\textbf{58.7} & 51.4 & \SetCell[c=1]{c, olive9}\textbf{60.4} & 56.2 & 55.0 & 56.9 & 94.2\\
& 8-S & 57.6 & 65.0 & \SetCell[c=1]{c, yellow9}\textbf{65.7} & \SetCell[c=1]{c, olive9}\textbf{66.6} & 62.6 & 63.7 & 63.6 & 56.1 & 65.0 & 62.7 & 94.7\\
& 8-M & 65.0 & \SetCell[c=1]{c, olive9}\textbf{68.9} & 67.2 & 65.5 & 61.6 & 66.4 & 56.9 & 66.7 & 63.4 & \SetCell[c=1]{c, yellow9}\textbf{67.7} & 95.0\\

\end{tblr}
}
\end{table*}

==> tables/map_12/map_moon.tex <==
\begin{table*}
\centering
\caption{Mean Average Precision (IOU=0.5) results (\%) for \textit{Moon}. Green indicates the highest-performing method for each YOLO model/size variant, where yellow and red represent the second and third highest respectively.}
\label{tab:map_moon}
\resizebox{\textwidth}{!}{%
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[1]Q[40]Q[50]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[50]},
  cells = {c},
  cell{1}{3} = {c=11}{},
  cell{2}{3} = {r=2}{},
  cell{2}{4} = {c=3}{},
  cell{2}{7} = {c=3}{},
  cell{2}{10} = {c=3}{},
  cell{2}{13} = {r=2}{},
  cell{4}{1} = {r=8}{},
  vline{3} = {4-11}{},
  vline{4,7,10,13} = {2-11}{dashed},
  hline{1} = {-}{},
  hline{3} = {4-12}{dashed},
  hline{4} = {3-13}{},
  hline{12} = {-}{},
}
 &  & \textbf{Method} &  &  &  &  &  &  &  &  &  & \\
 &  & {Source\\Only} & Adversarial &  &  & Contrastive &  &  & Full Feature &  &  & {Target\\Only}\\
 &  &  & ROI & Perceptual & Top-K & ROI & Perceptual & Top-K & YOCOv1 & K-Means & PTAP & \\
\begin{sideways}\textbf{Architecture}\end{sideways}

& 5-N & \SetCell[c=1]{c, olive9}\textbf{34.7} & 34.2 & 34.0 & \SetCell[c=1]{c, yellow9}\textbf{34.6} & 33.9 & 33.1 & 33.7 & 33.5 & \SetCell[c=1]{c, yellow9}\textbf{34.6} & \SetCell[c=1]{c, yellow9}\textbf{34.6} & 36.9\\
& 5-S & 33.9 & 34.6 & \SetCell[c=1]{c, yellow9}\textbf{34.9} & 33.4 & 34.6 & 33.8 & \SetCell[c=1]{c, olive9}\textbf{35.2} & 34.5 & 34.6 & 34.6 & 37.5\\
& 5-M & 34.7 & 34.0 & 33.9 & 34.0 & \SetCell[c=1]{c, yellow9}\textbf{35.1} & 34.1 & \SetCell[c=1]{c, olive9}\textbf{35.6} & 33.4 & 34.8 & 35.0 & 37.4\\
& 6-N & 34.0 & 33.4 & 33.7 & \SetCell[c=1]{c, yellow9}\textbf{34.4} & 33.3 & \SetCell[c=1]{c, yellow9}\textbf{34.4} & \SetCell[c=1]{c, olive9}\textbf{35.2} & 34.0 & 34.0 & 33.5 & 35.6\\
& 6-S & 33.6 & 34.5 & \SetCell[c=1]{c, yellow9}\textbf{35.1} & 34.8 & 34.1 & \SetCell[c=1]{c, olive9}\textbf{35.2} & 33.7 & 34.1 & 34.7 & 34.4 & 36.6\\
& 8-N & 33.4 & 33.7 & 34.2 & 33.7 & 33.5 & \SetCell[c=1]{c, olive9}\textbf{35.2} & \SetCell[c=1]{c, yellow9}\textbf{34.3} & 33.5 & 33.0 & 33.0 & 36.4\\
& 8-S & 33.0 & 33.6 & 33.6 & 32.9 & 32.3 & 33.8 & 33.3 & 33.9 & \SetCell[c=1]{c, olive9}\textbf{34.7} & \SetCell[c=1]{c, yellow9}\textbf{34.1} & 36.9\\
& 8-M & 32.8 & 33.2 & 33.9 & 33.1 & \SetCell[c=1]{c, olive9}\textbf{35.0} & \SetCell[c=1]{c, yellow9}\textbf{34.0} & 33.8 & 33.6 & 32.6 & 33.1 & 37.1\\

\end{tblr}
}
\end{table*}

==> tables/map_123/map_asteroid.tex <==
\begin{table*}
\centering
\caption{Mean Average Precision (IOU=0.5) results (\%) for \textit{Asteroid}. Green indicates the highest-performing method for each YOLO model/size variant, where yellow and red represent the second and third highest respectively.}
\label{tab:map_asteroid}
\resizebox{\textwidth}{!}{%
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[1]Q[40]Q[50]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[50]},
  cells = {c},
  cell{1}{3} = {c=11}{},
  cell{2}{3} = {r=2}{},
  cell{2}{4} = {c=3}{},
  cell{2}{7} = {c=3}{},
  cell{2}{10} = {c=3}{},
  cell{2}{13} = {r=2}{},
  cell{4}{1} = {r=8}{},
  vline{3} = {4-11}{},
  vline{4,7,10,13} = {2-11}{dashed},
  hline{1} = {-}{},
  hline{3} = {4-12}{dashed},
  hline{4} = {3-13}{},
  hline{12} = {-}{},
}
 &  & \textbf{Method} &  &  &  &  &  &  &  &  &  & \\
 &  & {Source\\Only} & Adversarial &  &  & Contrastive &  &  & Full Feature &  &  & {Target\\Only}\\
 &  &  & ROI & Perceptual & Top-K & ROI & Perceptual & Top-K & YOCOv1 & K-Means & PTAP & \\
\begin{sideways}\textbf{Architecture}\end{sideways}

& 5-N & \phantom{0}5.4 & 10.9 & \SetCell[c=1]{c, olive9}\textbf{53.1} & 15.0 & 37.6 & \SetCell[c=1]{c, brown9}\textbf{39.9} & 26.2 & 38.0 & 32.9 & \SetCell[c=1]{c, yellow9}\textbf{47.6} & 92.0\\
& 5-S & 35.5 & \SetCell[c=1]{c, yellow9}\textbf{56.5} & 44.7 & 34.9 & 37.2 & \SetCell[c=1]{c, brown9}\textbf{52.8} & 31.8 & 50.2 & \SetCell[c=1]{c, olive9}\textbf{57.0} & 35.7 & 92.4\\
& 5-M & 32.8 & 51.2 & \SetCell[c=1]{c, yellow9}\textbf{61.0} & \phantom{0}4.6 & 44.2 & 40.4 & \SetCell[c=1]{c, olive9}\textbf{61.2} & 44.7 & 49.5 & \SetCell[c=1]{c, brown9}\textbf{53.5} & 92.6\\
& 6-N & \SetCell[c=1]{c, brown9}\textbf{66.3} & 58.8 & 65.5 & 60.1 & 58.8 & 63.2 & 61.8 & \SetCell[c=1]{c, yellow9}\textbf{67.3} & \SetCell[c=1]{c, olive9}\textbf{67.4} & 62.8 & 91.9\\
& 6-S & 64.3 & 58.9 & \SetCell[c=1]{c, olive9}\textbf{66.2} & \SetCell[c=1]{c, yellow9}\textbf{65.7} & 58.9 & \SetCell[c=1]{c, brown9}\textbf{65.3} & 63.0 & 59.8 & 62.4 & 60.7 & 92.8\\
& 8-N & 26.0 & 31.1 & \SetCell[c=1]{c, brown9}\textbf{43.4} & \SetCell[c=1]{c, olive9}\textbf{60.7} & 40.3 & 17.8 & \SetCell[c=1]{c, yellow9}\textbf{55.3} & 34.0 & 43.3 & 24.1 & 91.8\\
& 8-S & \SetCell[c=1]{c, yellow9}\textbf{55.3} & 36.8 & \SetCell[c=1]{c, brown9}\textbf{55.2} & \SetCell[c=1]{c, olive9}\textbf{56.1} & 22.1 & 45.5 & 53.0 & \SetCell[c=1]{c, olive9}\textbf{56.1} & 13.2 & 18.7 & 92.5\\
& 8-M & 25.2 & 49.0 & \SetCell[c=1]{c, brown9}\textbf{49.5} & \SetCell[c=1]{c, olive9}\textbf{53.8} & 41.9 & 45.8 & 41.2 & \SetCell[c=1]{c, yellow9}\textbf{52.3} & 32.6 & 40.0 & 93.2\\

\end{tblr}
}
\end{table*}

==> tables/map_123/map_mars.tex <==
\begin{table*}
\centering
\caption{Mean Average Precision (IOU=0.5) results (\%) for \textit{Mars}. Green indicates the highest-performing method for each YOLO model/size variant, where yellow and red represent the second and third highest respectively.}
\label{tab:map_mars}
\resizebox{\textwidth}{!}{%
\begin{tblr}{
  width = \linewidth,
  % Used to be 60s
  colspec = {Q[1]Q[40]Q[50]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[50]},
  cells = {c},
  cell{1}{3} = {c=11}{},
  cell{2}{3} = {r=2}{},
  cell{2}{4} = {c=3}{},
  cell{2}{7} = {c=3}{},
  cell{2}{10} = {c=3}{},
  cell{2}{13} = {r=2}{},
  cell{4}{1} = {r=8}{},
  vline{3} = {4-11}{},
  vline{4,7,10,13} = {2-11}{dashed},
  hline{1} = {-}{},
  hline{3} = {4-12}{dashed},
  hline{4} = {3-13}{},
  hline{12} = {-}{},
}
 &  & \textbf{Method} &  &  &  &  &  &  &  &  &  & \\
 &  & {Source\\Only} & Adversarial &  &  & Contrastive &  &  & Full Feature &  &  & {Target\\Only}\\
 &  &  & ROI & Perceptual & Top-K & ROI & Perceptual & Top-K & YOCOv1 & K-Means & PTAP & \\
\begin{sideways}\textbf{Architecture}\end{sideways}

& 5-N & 51.1 & 57.9 & 55.7 & \SetCell[c=1]{c, olive9}\textbf{62.4} & 56.4 & 53.6 & 52.2 & \SetCell[c=1]{c, yellow9}\textbf{59.3} & 54.3 & \SetCell[c=1]{c, brown9}\textbf{58.4} & 93.7\\
& 5-S & 64.0 & \SetCell[c=1]{c, yellow9}\textbf{65.4} & 64.0 & \SetCell[c=1]{c, brown9}\textbf{64.6} & 60.7 & 60.9 & \SetCell[c=1]{c, olive9}\textbf{66.3} & 62.7 & 55.5 & 63.2 & 94.2\\
& 5-M & 63.2 & 68.3 & \SetCell[c=1]{c, yellow9}\textbf{71.4} & 66.1 & \SetCell[c=1]{c, olive9}\textbf{71.6} & 65.9 & 68.4 & \SetCell[c=1]{c, brown9}\textbf{68.8} & 65.4 & 62.9 & 94.9\\
& 6-N & \SetCell[c=1]{c, yellow9}\textbf{64.9} & 58.2 & 56.7 & 56.1 & 55.2 & 59.2 & 55.8 & \SetCell[c=1]{c, olive9}\textbf{65.0} & \SetCell[c=1]{c, brown9}\textbf{60.4} & 50.8 & 93.9\\
& 6-S & 60.9 & 64.3 & 66.0 & 64.3 & 65.7 & \SetCell[c=1]{c, yellow9}\textbf{69.2} & \SetCell[c=1]{c, olive9}\textbf{69.6} & 65.5 & \SetCell[c=1]{c, brown9}\textbf{66.2} & 64.2 & 94.3\\
& 8-N & \SetCell[c=1]{c, brown9}\textbf{57.4} & 51.9 & 55.9 & 51.7 & \SetCell[c=1]{c, yellow9}\textbf{58.7} & 51.4 & \SetCell[c=1]{c, olive9}\textbf{60.4} & 56.2 & 55.0 & 56.9 & 94.2\\
& 8-S & 57.6 & \SetCell[c=1]{c, brown9}\textbf{65.0} & \SetCell[c=1]{c, yellow9}\textbf{65.7} & \SetCell[c=1]{c, olive9}\textbf{66.6} & 62.6 & 63.7 & 63.6 & 56.1 & \SetCell[c=1]{c, brown9}\textbf{65.0} & 62.7 & 94.7\\
& 8-M & 65.0 & \SetCell[c=1]{c, olive9}\textbf{68.9} & \SetCell[c=1]{c, brown9}\textbf{67.2} & 65.5 & 61.6 & 66.4 & 56.9 & 66.7 & 63.4 & \SetCell[c=1]{c, yellow9}\textbf{67.7} & 95.0\\

\end{tblr}
}
\end{table*}

==> tables/map_123/map_moon.tex <==
\begin{table*}
\centering
\caption{Mean Average Precision (IOU=0.5) results (\%) for \textit{Moon}. Green indicates the highest-performing method for each YOLO model/size variant, where yellow and red represent the second and third highest respectively.}
\label{tab:map_moon}
\resizebox{\textwidth}{!}{%
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[1]Q[40]Q[50]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[75]Q[50]},
  cells = {c},
  cell{1}{3} = {c=11}{},
  cell{2}{3} = {r=2}{},
  cell{2}{4} = {c=3}{},
  cell{2}{7} = {c=3}{},
  cell{2}{10} = {c=3}{},
  cell{2}{13} = {r=2}{},
  cell{4}{1} = {r=8}{},
  vline{3} = {4-11}{},
  vline{4,7,10,13} = {2-11}{dashed},
  hline{1} = {-}{},
  hline{3} = {4-12}{dashed},
  hline{4} = {3-13}{},
  hline{12} = {-}{},
}
 &  & \textbf{Method} &  &  &  &  &  &  &  &  &  & \\
 &  & {Source\\Only} & Adversarial &  &  & Contrastive &  &  & Full Feature &  &  & {Target\\Only}\\
 &  &  & ROI & Perceptual & Top-K & ROI & Perceptual & Top-K & YOCOv1 & K-Means & PTAP & \\
\begin{sideways}\textbf{Architecture}\end{sideways}

& 5-N & \SetCell[c=1]{c, olive9}\textbf{34.7} & \SetCell[c=1]{c, brown9}\textbf{34.2} & 34.0 & \SetCell[c=1]{c, yellow9}\textbf{34.6} & 33.9 & 33.1 & 33.7 & 33.5 & \SetCell[c=1]{c, yellow9}\textbf{34.6} & \SetCell[c=1]{c, yellow9}\textbf{34.6} & 36.9\\
& 5-S & 33.9 & \SetCell[c=1]{c, brown9}\textbf{34.6} & \SetCell[c=1]{c, yellow9}\textbf{34.9} & 33.4 & \SetCell[c=1]{c, brown9}\textbf{34.6} & 33.8 & \SetCell[c=1]{c, olive9}\textbf{35.2} & 34.5 & \SetCell[c=1]{c, brown9}\textbf{34.6} & \SetCell[c=1]{c, brown9}\textbf{34.6} & 37.5\\
& 5-M & 34.7 & 34.0 & 33.9 & 34.0 & \SetCell[c=1]{c, yellow9}\textbf{35.1} & 34.1 & \SetCell[c=1]{c, olive9}\textbf{35.6} & 33.4 & 34.8 & \SetCell[c=1]{c, brown9}\textbf{35.0} & 37.4\\
& 6-N & \SetCell[c=1]{c, brown9}\textbf{34.0} & 33.4 & 33.7 & \SetCell[c=1]{c, yellow9}\textbf{34.4} & 33.3 & \SetCell[c=1]{c, yellow9}\textbf{34.4} & \SetCell[c=1]{c, olive9}\textbf{35.2} & \SetCell[c=1]{c, brown9}\textbf{34.0} & \SetCell[c=1]{c, brown9}\textbf{34.0} & 33.5 & 35.6\\
& 6-S & 33.6 & 34.5 & \SetCell[c=1]{c, yellow9}\textbf{35.1} & \SetCell[c=1]{c, brown9}\textbf{34.8} & 34.1 & \SetCell[c=1]{c, olive9}\textbf{35.2} & 33.7 & 34.1 & 34.7 & 34.4 & 36.6\\
& 8-N & 33.4 & 33.7 & \SetCell[c=1]{c, brown9}\textbf{34.2} & 33.7 & 33.5 & \SetCell[c=1]{c, olive9}\textbf{35.2} & \SetCell[c=1]{c, yellow9}\textbf{34.3} & 33.5 & 33.0 & 33.0 & 36.4\\
& 8-S & 33.0 & 33.6 & 33.6 & 32.9 & 32.3 & 33.8 & 33.3 & \SetCell[c=1]{c, brown9}\textbf{33.9} & \SetCell[c=1]{c, olive9}\textbf{34.7} & \SetCell[c=1]{c, yellow9}\textbf{34.1} & 36.9\\
& 8-M & 32.8 & 33.2 & \SetCell[c=1]{c, brown9}\textbf{33.9} & 33.1 & \SetCell[c=1]{c, olive9}\textbf{35.0} & \SetCell[c=1]{c, yellow9}\textbf{34.0} & 33.8 & 33.6 & 32.6 & 33.1 & 37.1\\

\end{tblr}
}
\end{table*}
